Beyond the Broadcast: Enhancing VR Tennis Broadcasting through Embedded Visualizations and Camera Techniques

Virtual Reality (VR) broadcasting has emerged as a promising medium for providing immersive viewing experiences of major sports events such as tennis. However, current VR broadcast systems often lack an effective camera language and do not adequately incorporate dynamic, in-game visualizations, limiting viewer engagement and narrative clarity. To address these limitations, we analyze 400 out-of-play segments from eight major tennis broadcasts to develop a tennis-specific design framework that effectively combines cinematic camera movements with embedded visualizations. We further refine our framework by examining 25 cinematic VR animations, comparing their camera techniques with traditional tennis broadcasts to identify key differences and inform adaptations for VR. Based on data extracted from the broadcast videos, we reconstruct a simulated game that captures the players' and ball's motion and trajectories. Leveraging this design framework and processing pipeline, we develope Beyond the Broadcast, a VR tennis viewing system that integrates embedded visualizations with adaptive camera motions to construct a comprehensive and engaging narrative. Our system dynamically overlays tactical information and key match events onto the simulated environment, enhancing viewer comprehension and narrative engagement while ensuring perceptual immersion and viewing comfort. A user study involving tennis viewers demonstrate that our approach outperforms traditional VR broadcasting methods in delivering an immersive, informative viewing experience.

==> README <==
Created by Torsten Moeller, April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016
modified by Cagatay Turkay and Soumya Dutta, September 2019
modified by Cody Dunne, January and March 2023

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used with an established LaTeX environment by calling pdfLaTeX or LaTex. For online collaborative editing or without a local LaTeX installation, one option is to use https://www.overleaf.com/. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Unix-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> Section/6-Discussion.tex <==
% \section{Discussion}\label{sec-6}

% \textbf{Balancing Presence and Immersion.}
% % Our findings reveal a critical trade-off between perceptual immersion (objective system fidelity) and subjective presence (users’ felt “being there”). While increasing visual realism and dynamic camera motion can heighten presence, it may also overload viewers’ cognitive resources and impede comprehension. This aligns with Skarbez et al.’s survey of presence concepts, which cautions that excessive sensory detail can detract from cognitive processing of task-relevant information [Skarbez et al. 2017]. Designers must therefore navigate this tension by calibrating visual and interaction fidelity to support both immersion and understanding.


% \textbf{Narrative vs. Perceptual Immersion.}
% % We observed that narrative immersion—through well-timed camera language and embedded storytelling cues—can compensate for limitations in perceptual fidelity. Consistent with Ryan’s theory of narrative virtual reality, structuring camera transitions and data overlays around core events fosters a coherent story experience, even when photorealism is constrained [Ryan 2001]. In practice, emphasizing narrative engagement (e.g., “forced perspective” visualizations) can be more effective than pursuing marginal gains in graphical realism.


% \textbf{Attention Management in VR.}
% % Embedded visualizations must guide rather than distract. Progressive disclosure—revealing tactical data only at pivotal moments—helps prevent cognitive overload. Prouzeau et al. show that attention-aware displays can dynamically adapt information density based on user focus [Prouzeau et al. 2024]. Our results suggest a similar strategy: start with minimal overlays, then gradually layer in details as viewers’ attention stabilizes.

% \textbf{Comfort–Engagement Trade-offs.}
% % Seated viewing paradigms significantly reduce fatigue while preserving analytical capacity, as demonstrated by VirtualDesk’s comfortable immersive displays [Wagner Filho et al. 2018]. In our study, participants reported higher comfort during stabilized, baseline viewpoints, yet they found dynamic shots more engaging. This underscores the need for hybrid approaches—anchoring users in a comfortable posture while intermittently introducing motion to sustain interest.


% \textbf{VR as a New Narrative Medium.}
% % Unlike 2D broadcasts—which simply extend existing camera angles—VR demands a reimagining of narrative structure. Information density and timing must be adapted to 6 DoF viewing, balancing user control with guided storytelling. Viewers can no longer passively absorb a single fixed frame; they require cues that anchor their gaze and convey narrative priority.


% \textbf{Generalizability to Other Sports.}
% % Our design framework is tailored to tennis’s one-on-one dynamics and linear ball trajectories. Team sports (e.g., basketball or soccer) introduce multi-agent interactions and more complex tactical overlays, necessitating new tracking methods and narrative schemas. Adapting the framework will require sport-specific camera grammars and embedded-visualization strategies to manage increased visual complexity.


% \textbf{Adaptive Personalization.}
% % Individual viewers differ in expertise and susceptibility to cybersickness. Future systems should learn each user’s comfort threshold and tennis knowledge—automatically adjusting camera smoothness, overlay density, and pacing accordingly [Caserman et al. 2021]. Such adaptive personalization can optimize both engagement and comfort.


% \textbf{Multimodal Enhancement.}
% % To approximate the live-match ambiance, VR broadcasts should integrate spatial audio (crowd reactions, on-court commentary) and event-driven haptic feedback (e.g., subtle vibrations on key serves). Thoughtful multimodal fusion can enrich presence without overloading any single sensory channel, creating a more holistic and socially resonant experience.


% % cognitive attention and Embedded visualizations
% % Attention-Aware Visualization: Tracking and Responding to User Perception Over Time

% % Research demonstrates that spatial integration of information within the virtual environment reduces cognitive load compared to overlay interfaces. 




% % narrative engagement and perceptual immersion trade-offs 
% % RetroSketch: A Retrospective Method for Measuring Emotions
% % and Presence in Virtual Reality
% % Content design strategies should emphasize narrative immersion elements that can compensate for technical limitations, spatial integration of statistical and supplementary information rather than overlay approaches, and progressive disclosure of complexity based on user expertise and engagement.
% % There is nothing virtual about immersion: Narrative immersion for VR and other interfaces
% % Grammar of VR Storytelling: Narrative Immersion and
% % Experiential Fidelity in VR Cinema


% % Visual realism vs information visualization trade-offs
% % Perspective: Does Realism Improve Presence in VR? Suggesting a Model and Metric for VR Experience Evaluation

% % "While embedded visualizations disrupt photorealism (e.g., ball trails), they amplify narrative clarity by guiding attention—similar to 'forced perspective' in cinema [40]. This aligns with Bressa et al. [4]: 'Situated visualizations prioritize function over fidelity'."



% % Camera motion principles for minimizing sickness
% % "Slow linear motions (avg. 0.5m/s) minimized discomfort vs. rapid pans (＞30°/s) causing 2/16 viewers nausea—supporting Zhu et al. [82]'s 'velocity threshold model'."



% % Balance comfort and engagement
% % VirtualDesk: A Comfortable and Efficient Immersive Information Visualization Approach
% % Presence and Cybersickness in Virtual Reality Are Negatively Related: A Review

% % The seated experience principle emerges strongly from multiple studies: seated interactions for information-intensive tasks significantly reduce fatigue while maintaining analytical effectiveness. Sports broadcasts could implement stadium seating metaphors that provide comfort boundaries while enabling immersive viewing.


% % User agency needed? Can discuss in the future work session
% % Passive viewing experiences show higher motion sickness rates and lower presence compared to interactive approaches.
% % A review of cybersickness in head‑mounted displays: raising attention to individual susceptibility
% % Sports broadcasts should provide meaningful interaction opportunities—camera angle selection, information access, social features—while maintaining comfortable defaults for passive viewers.


% % Multimodal feedback integration
% % Combining visual, auditory, and haptic feedback enhances understanding and engagement without overwhelming individual sensory channels. Sports applications could leverage spatial audio for crowd atmosphere, haptic feedback for key moments, and visual highlighting for important game elements.


% % Implications for VR sports broadcasting
% % "Framework applicable to net sports (badminton/pickleball) with court geometry adaptation, but team sports require multi-agent tracking (see Limitation 7.2)"




==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)

